Pedagogical Alignment of Large Language Models

Large Language Models (LLMs), when used in educational settings without pedagogical fine-tuning, often provide immediate answers rather than guiding students through the problem-solving process. This approach falls short of pedagogically best practices and limits their effectiveness as educational tools. We term the objective of training LLMs to emulate effective teaching strategies as `pedagogical alignment.' In this paper, we investigate Learning from Human Preferences (LHP) algorithms to achieve this alignment objective. A key challenge in this process is the scarcity of high-quality preference datasets to guide the alignment. To address this, we propose a novel approach for constructing a large-scale dataset using synthetic data generation techniques, eliminating the need for time-consuming and costly manual annotation. Leveraging this dataset, our experiments with Llama and Mistral models demonstrate that LHP methods outperform standard supervised fine-tuning (SFT), improving pedagogical alignment accuracy by 13.1% and 8.7% respectively. Existing evaluation methods also lack quantitative metrics to adequately measure the pedagogical alignment of LLMs. To address this gap, we propose novel perplexity-based metrics that quantify LLMs' tendency to provide scaffolded guidance versus direct answers, offering a robust measure of pedagogical alignment. Our analysis provides compelling evidence for the superiority of LHP methods over SFT in optimizing LLMs' behavior, underscoring the potential of LHP methods in better aligning LLMs with educational objectives and fostering effective learning experiences. Code and models are available \href{https://github.com/luffycodes/Tutorbot-Spock}{here}.

==> tables/openllm.tex <==
\begin{table}[t!]
\caption{LLM Performance on key benchmarks. This table presents the performance of Mistral, Zephyr, and Vicuna on different NLP benchmarks \citep{eval-harness}.
% \citep{open-llm-leaderboard,eval-harness,clark2018think,zellers2019hellaswag,hendrycks2021measuring,lin2022truthfulqa,DBLP:journals/corr/abs-1907-10641,DBLP:journals/corr/abs-2110-14168}
We selected Mistral and Zephyr based on their superior performance across various benchmarks, which provided a thorough assessment across a spectrum of reasoning and general knowledge tasks.
We chose Vicuna because it served as the base model for the CLASS framework.}
\label{tab:leaderboard}
\centering
\resizebox{\columnwidth}{!}{
\begin{tabular}{|l|c|c|c|c|c|c|c|}
\hline
\textbf{Model}                    & \textbf{Average} & \textbf{ARC}   & \textbf{HellaSwag} & \textbf{MMLU}  & \textbf{TruthfulQA} & \textbf{Winogrande} & \textbf{GSM8K} \\ \hline
Mistral & \textbf{65.71}   & \textbf{63.14} & \textbf{84.88}     & 60.78 & \textbf{68.26}      & 77.19      & \textbf{40.03} \\ 
Zephyr            & 61.95   & 62.03 & 84.36     & \textbf{61.07} & 57.45      & \textbf{77.74}      & 29.04 \\ 
Vicuna           & 52.06   & 53.24 & 77.39     & 50.82 & 50.33      & 72.06      & 8.11  \\ \hline
\end{tabular}}
\end{table}


==> tables/rlhf_results_v2.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table}[t!]
\caption{}
\label{tab:my-table}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{|l|ccc|ccc|ccc|ccc|}
\hline
Model/Algorithm & \multicolumn{3}{c|}{\textbf{SFT}} & \multicolumn{3}{c|}{\textbf{DPO}} & \multicolumn{3}{c|}{\textbf{IPO}} & \multicolumn{3}{c|}{\textbf{KTO}} \\ \hline
\textbf{} &
  \multicolumn{1}{l|}{E} &
  \multicolumn{1}{l|}{A} &
  S &
  \multicolumn{1}{c|}{E} &
  \multicolumn{1}{c|}{A} &
  S &
  \multicolumn{1}{c|}{E} &
  \multicolumn{1}{c|}{A} &
  S &
  \multicolumn{1}{c|}{E} &
  \multicolumn{1}{c|}{A} &
  S \\
\textbf{Mistral-7B-instruct} &
  \multicolumn{1}{c|}{34} &
  \multicolumn{1}{c|}{34} &
  37 &
  \multicolumn{1}{c|}{72} &
  \multicolumn{1}{c|}{72} &
  78 &
  \multicolumn{1}{c|}{56} &
  \multicolumn{1}{c|}{56} &
  61 &
  \multicolumn{1}{c|}{73} &
  \multicolumn{1}{c|}{73} &
  80 \\
\textbf{vicuna-7b-v1.5} &
  \multicolumn{1}{c|}{73} &
  \multicolumn{1}{c|}{70} &
  80 &
  \multicolumn{1}{c|}{73} &
  \multicolumn{1}{c|}{72} &
  80 &
  \multicolumn{1}{c|}{74} &
  \multicolumn{1}{c|}{72} &
  82 &
  \multicolumn{1}{c|}{73} &
  \multicolumn{1}{c|}{72} &
  81 \\
\textbf{zephy-7b-beta} &
  \multicolumn{1}{c|}{12} &
  \multicolumn{1}{c|}{11} &
  9 &
  \multicolumn{1}{c|}{72} &
  \multicolumn{1}{c|}{71} &
  79 &
  \multicolumn{1}{c|}{22} &
  \multicolumn{1}{c|}{22} &
  21 &
  \multicolumn{1}{c|}{73} &
  \multicolumn{1}{c|}{72} &
  79 \\ \hline
\end{tabular}%
}
\end{table}
